Networks of UAVs of Low-Complexity for Time-Critical Localization

Future networks of unmanned aerial vehicles (UAVs) will be tasked to carry out ever-increasing complex operations that are time-critical and that require accurate localization performance (e.g., tracking the state of a malicious user). Since there is the need to preserve low UAV complexity while tackling the challenging goals of missions in effective ways, one key aspect is the UAV intelligence (UAV-I). The UAV's intelligence includes the UAV's capability to process information and to make decisions, e.g., to decide where to sense and whether to delegate some tasks to other network entities. In this paper, we provide an overview of possible solutions for the design of UAVs of low complexity, showing some of the needs of the UAVs for running efficient localization operations, performed either as a team or individually. Further, we focus on different network configurations, which possibly include assistance with edge computing. We also discuss open problems and future perspectives for these settings.

==> AESS Magazine - UAV/acronyms.tex <==
%Numbers
\acrodef{5G}{fifth generation}
\acrodef{6G}{sixth generation}
%A
\acrodef{AI}{artificial intelligence}
\acrodef{UAV-I}{{\em UAV intelligence}}
\acrodef{AI/ML}{artificial intelligence/machine learning}
\acrodef{CNPC}{control and non-payload communication}
\acrodef{A2A}{agent-to-agent}
\acrodef{AWGN}{additive white Gaussian noise}
%B
\acrodef{BS}{base station}
%C
\acrodef{CRLB}{Cram\'er-Rao Lower Bound}
\acrodef{CDF}{cumulative density function}
\acrodef{CDR}{correct detection rate}
\acrodef{CIR}{channel impulse response}
\acrodef{CRAS}{connected robotics and autonomous systems}
%D
\acrodef{DEC-POMDP}{decentralized partially observable Markov decision process}
\acrodef{D2D}{device-to-device}
%E
\acrodef{EKF}{extended Kalman filter}
\acrodef{EIRP}{effective isotropic radiated power}
\acrodef{KF}{Kalman filter}
%F
\acrodef{FAR}{false alarm rate}
\acrodef{FIM}{Fisher Information matrix}
\acrodef{FL}{federated learning}
\acrodef{FMCW}{frequency modulated continuous wave}
%G
\acrodef{GLRT}{generalized likelihood ratio test}
\acrodef{GP}{Gaussian process}
\acrodef{GPI}{generalized policy iteration}
%I
\acrodef{IoT}{Internet-of-Things}
\acrodef{IS}{image similarity}
%K
\acrodef{KPI}{key performance indicator}
%L
\acrodef{LLRT}{log-likelihood ratio test}
\acrodef{LOS}{line-of-sight}
%M
 \acrodef{MAC}{medium access control}
\acrodef{MAP}{maximum a-posteriori probability}
\acrodef{MEC}{multi-access edge computing}
\acrodef{mMTC}{massive machine type communication}
\acrodef{eMBB}{enhanced mobile broadband}


\acrodef{MMSE}{minimum mean squared error }
\acrodef{MARL}{multi-agent reinforcement learning}
\acrodef{MDP}{Markov decision process}
\acrodef{MIMO}{multiple input multiple output}
\acrodef{ML}{machine learning}
\acrodef{MLE}{maximum likelihood estimator}
\acrodef{mm-wave}{millimeter-wave}
%N
\acrodef{NOMA}{non-orthogonal multiple access}
\acrodef{NLOS}{non line-of-sight}
%O
\acrodef{OG}{occupancy grid}
%P
\acrodef{PF}{particle filtering}
\acrodef{pdf}{probability density function}
\acrodef{PFA}{probability of false alarm}
\acrodef{PL}{packet loss}
\acrodef{POMDP}{partially observable Markov decision process}
\acrodef{PER}{packet error rate}
%R
\acrodef{RCS}{radar cross section}
\acrodef{RMSE}{root mean square error}
\acrodef{RFID}{radiofrequency identification}
\acrodef{RL}{reinforcement learning}
\acrodef{ROC}{receiver operating characteristics}
\acrodef{RR}{reading range}
\acrodef{RRCS}{root-radar cross section}
\acrodef{RV}{random variable}
%S
\acrodef{SLAM}{simultaneous localization and mapping}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{SIR}{sequential importance resampling} 
%T
\acrodef{TD}{temporal-difference}
%U
\acrodef{THz}{Terahertz}
\acrodef{UAV}{unmanned aerial vehicle}
\acrodef{U2U}{UAV-to-UAV}
\acrodef{UKF}{Unscented Kalman Filter}
\acrodef{URLLC}{ultrareliable and low-latency communication}
%V
\acrodef{VLC}{visible light communication}


